Minimising the expectation value of the procurement cost in electricity markets based on the prediction error of energy consumption

In this paper, we formulate a method for minimising the expectation value of the procurement cost of electricity in two popular spot markets: {\it day-ahead} and {\it intra-day}, under the assumption that expectation value of unit prices and the distributions of prediction errors for the electricity demand traded in two markets are known. The expectation value of the total electricity cost is minimised over two parameters that change the amounts of electricity. Two parameters depend only on the expected unit prices of electricity and the distributions of prediction errors for the electricity demand traded in two markets. That is, even if we do not know the predictions for the electricity demand, we can determine the values of two parameters that minimise the expectation value of the procurement cost of electricity in two popular spot markets. We demonstrate numerically that the estimate of two parameters often results in a small variance of the total electricity cost, and illustrate the usefulness of the proposed procurement method through the analysis of actual data.

==> ref.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%
%Mamoru Imanishi         %
%http://www.okomeda.net/ %
%%%%%%%%%%%%%%%%%%%%%%%%%%

@misc{Agency, 
author={Agency for Natural Resources and Energy}, 
title={Overview of the Present Situation Regarding Imbalance Fees (in Japanese)}, 
howpublished={http://www.meti.go.jp{\slash}committee{\slash}sougouenergy{\slash}denryoku\_gas{\slash}denryoku\_gas\_kihon{\slash}seido\_kento{\slash}pdf{\slash}007\_04\_00.pdf}
}

@article{bathurst2002trading,
  title={Trading wind generation in short term energy markets},
  author={Bathurst, Graeme N and Weatherill, Jennie and Strbac, Goran},
  journal={IEEE Transactions on Power Systems},
  volume={17},
  number={3},
  pages={782--789},
  year={2002},
  publisher={IEEE}
}

@inproceedings{chinnathambi2016investigation,
author={R. A. Chinnathambi and P. Ranganathan}, 
booktitle={2016 IEEE International Conference on Big Data (Big Data)}, 
title={Investigation of forecasting methods for the hourly spot price of the day-ahead electric power markets}, 
year={2016}, 
volume={}, 
number={}, 
pages={3079-3086}, 
keywords={autoregressive moving average processes;load forecasting;power engineering computing;power markets;support vector machines;forecasting methods;hourly spot price;day-ahead electric power markets;Iberian electricity market;MIBEL;mean absolute percentage error;MAPE;autoregressive integrated moving average;ARIMA;generalized linear model;GLM;random forest;support vector machines;SVM methods;Predictive models;Support vector machines;Computational modeling;Electricity supply industry;Forecasting;Data models;Load modeling;ARIMA-GLM;Hybrid model;Generalized Linear Model;Electricity Price Forecasting;Random Forest;Support Vector Machine;Iberian Market;Day -ahead Price}, 
doi={10.1109/BigData.2016.7840962}, 
ISSN={}, 
month={Dec},}

@article{srinivasan2016bidding,
  title={Bidding and cooperation strategies for electricity buyers in power markets},
  author={Srinivasan, Dipti and Trung, Ly Trong and Singh, Chanan},
  journal={IEEE Systems Journal},
  volume={10},
  number={2},
  pages={422--433},
  year={2016},
  publisher={IEEE}
}

@book{hiroakinagayama2013,
	author	= {Hiroaki Nagayama},
	title	= {Political economics of the unbundling of electricity generation and transmission (in Japanese)},
	publisher = {Toyokeizaishinpo-sha},
	year	= {2012},
	address = {}
}

@techreport{techrepo2016,
	author={Investigating R\&D Committee on Recommended Practice for Simulation Models for Automatic Generation Control}, 
	title={``Recommended Practice for Simulation Models for Automatic Generation Control,'' Technical Report (in Japanese)}, 
	institution={The Institute of Electrical Engineers of Japan}, 
	year={2016}, 
	volume={1386}
}

@misc{JEPX, 
author={Japan Electric Power eXchange}, 
title={Japan Electric Power eXchange Guide (in Japanese)}, 
howpublished={http://www.jepx.org{\slash}outline{\slash}pdf{\slash}Guide\_2.00.pdf}
}

@inproceedings{li2015optimal,
author={J. Li and Z. Li and Y. Wang}, 
booktitle={2015 North American Power Symposium (NAPS)}, 
title={Optimal bidding strategy for day-ahead power market}, 
year={2015}, 
volume={}, 
number={}, 
pages={1-6}, 
keywords={game theory;optimisation;power generation economics;power markets;power transmission economics;pricing;profitability;tendering;day-ahead power market auction;optimal bidding strategy;generation companies;electric power market;bid generation price;bid curve;supply curve segment;intertemporal physical constraint;multiple period bidding strategy;noncooperative game;two-layer optimization problem;GENCO profit maximization problem;independent system operator;ISO market clearing problem;transmission constrained market clearing;Games;Power markets;Cost function;ISO;Companies;Generators;Silicon;Imperfect competition;non-cooperative game;day-ahead power market;GENCO;Incomplete information game;Conditional profit}, 
doi={10.1109/NAPS.2015.7335133}, 
ISSN={}, 
month={Oct},}

@article{miyauchi2014regression,
  title={Regression analysis of electric power market price of JEPX},
  author={Miyauchi, Hajime and Misawa, Tetsuya},
  journal={Journal of Power and Energy Engineering},
  volume={2},
  number={04},
  pages={483},
  year={2014},
  publisher={Scientific Research Publishing}
}

@article{matevosyan2006minimization,
  title={Minimization of imbalance cost trading wind power on the short-term power market},
  author={Matevosyan, Julija and Soder, Lennart},
  journal={IEEE Transactions on Power Systems},
  volume={21},
  number={3},
  pages={1396--1404},
  year={2006},
  publisher={IEEE}
}

@inproceedings{ofuji2007price,
booktitle={2007 International Conference on Intelligent Systems Applications to Power Systems}, 
title={Price Forecasting of Japan Electric Power Exchange using Time-varying AR Model}, 
year={2007}, 
volume={}, 
number={}, 
pages={1-6}, 
keywords={least squares approximations;maximum likelihood estimation;power markets;power system economics;recursive estimation;price forecasting;Japan Electric Power Exchange;time-varying AR model;spot market;price time series;market dynamics;stepwise recursive estimation;Kalman filter algorithm;maximum likelihood method;spot electricity strip price;ordinary least square method;Predictive models;Economic forecasting;Recursive estimation;State-space methods;Time series analysis;Optimization methods;Maximum likelihood estimation;Strips;Econometrics;Yield estimation;Japan Electric Power Exchange(JEPX);Day-ahead spot market;Price forecasting;Time-series decomposition;Kalman Filter algorithm}, 
doi={10.1109/ISAP.2007.4441658}, 
ISSN={}, 
month={Nov},}

@article{girish2016spot,
  title={Spot electricity price forecasting in Indian electricity market using autoregressive-GARCH models},
  author={Girish, GP},
  journal={Energy Strategy Reviews},
  volume={11},
  pages={52--57},
  year={2016},
  publisher={Elsevier}
}

@article{voronin2013price,
  title={Price forecasting in the day-ahead energy market by an iterative method with separate normal price and price spike frameworks},
  author={Voronin, Sergey and Partanen, Jarmo},
  journal={Energies},
  volume={6},
  number={11},
  pages={5897--5920},
  year={2013},
  publisher={Multidisciplinary Digital Publishing Institute}
}

@book{fahrmeir2013regression,
  title={Regression: models, methods and applications},
  author={Fahrmeir, Ludwig and Kneib, Thomas and Lang, Stefan and Marx, Brian},
  year={2013},
  publisher={Springer Science \& Business Media}
}


%%%%% article %%%%%
@article{ mye:1981,
	author	= {Roger B. Myerson},
	title 	= {Optimal Auction Design},
	journal	= {Mathematics of Operations Research},
	year	= {1981},
	volume	= {6},
	number	= {1},
	month	= {feb},
	pages	= {58-73}
}
@article{das:1979,
	author	= {Partha Dasgupta and Peter Hammond and Eric Maskin},
	title	= {The Implemntation of Social Choice Rules: Some General Results on Incentive Compatibility},
	journal	= {Review of Economic Studies},
    	year	= {1979},
	volume	= {46},
    	pages	= {185-216}
}
@article{laf:1980,
	author	= {Jean-Jacques Laffont and Eric Maskin},
	title	= {A Differential Approach to Dominant Strategy Mechanisms},
        journal	= {Econometrica},
	year	= {1980},
	volume	= {48},
	pages	= {1507-1520}
}

@article{sjo:1996a,
	author	= {Tomas Sj{\"o}str{\"o}m},
	title	= {Implementation and Information in Teams},
	journal = {Economic Design},
	year	= {1996},
	volume	= {1},
    	pages	= {327-341}
}

@article{sjo:1996b,
	author	= {Tomas Sj{\"o}str{\"o}m},
	title	= {Implementation by Demand Mechanisms},
	journal = {Economic Design},
	year	= {1996},
	volume	= {1},    	
    	pages	= {343-354}
}




%%%%% book %%%%%
@book{ red:2003,
	author	= {Fernand Vega-Redondo},
	title	= {Economics and the Theory of Games},
	publisher = {Cambridge University Press},
	year	= {2003},
	address = {Cambridge}
}
@book{mye:1991,
	author	= {Roger B. Myerson},
   	title	= {Game Theory: Analysis of Conflict},
   	address = {Cambridge},
  	publisher = {Harvard University Press},
	 year	= {1991}
}
%%%%% inbook %%%%%
@inbook{ mas:1995,
	author	= {Andreu Mas-Corell and Michael Winston and Jerry Green},
    	title	= {Microeconomic Theory},
	year	= {1995},
    	address	= {Oxford},
    	publisher= {Oxford University Press},
	chapter	= {13,14},
	pages	= {436-510}
}
%%%%% incollection %%%%%
@incollection{ mas:1985,
   	author	= {Eric Maskin},
    	title	= {The Theory of Implementation in Nash Equilibrium: A Survey},
    	booktitle = {Social Goals And Social Organization},
    	editor	= {Leonid Hurwicz and David Schmeidler and Hugo Sonnenschein},
    	year	= {1985},
    	address = {Cambridge},
    	publisher = {Cambridge Unviersity Press},
    	pages	= {173-204}
}
